VQA-based Robotic State Recognition Optimized with Genetic Algorithm

State recognition of objects and environment in robots has been conducted in various ways. In most cases, this is executed by processing point clouds, learning images with annotations, and using specialized sensors. In contrast, in this study, we propose a state recognition method that applies Visual Question Answering (VQA) in a Pre-Trained Vision-Language Model (PTVLM) trained from a large-scale dataset. By using VQA, it is possible to intuitively describe robotic state recognition in the spoken language. On the other hand, there are various possible ways to ask about the same event, and the performance of state recognition differs depending on the question. Therefore, in order to improve the performance of state recognition using VQA, we search for an appropriate combination of questions using a genetic algorithm. We show that our system can recognize not only the open/closed of a refrigerator door and the on/off of a display, but also the open/closed of a transparent door and the state of water, which have been difficult to recognize.

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag} % 古いコマンドやパッケージの利用を警告する
\usepackage[all, warning]{onlyamsmath} % amsmath が提供しない数式環境を使用した場合に警告
\usepackage{hyperref}
\usepackage{color}
\usepackage{graphicx}
\usepackage{url}

%%%% カスタマイズしたい場合は以下に書く

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}

% hypcap: figref, tabrefしたときにジャンプ先がキャプション部ではなく図の上になる
\usepackage[figure,figure*,table,table*]{hypcap}
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}

\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}

\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\tabref}[1]{{Table \ref{#1}}}
\newcommand{\figref}[1]{{Fig. \ref{#1}}}
\newcommand{\equref}[1]{{Eq. \ref{#1}}}
\newcommand{\algoref}[1]{{Alg. \ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}

